Self-Training Large Language Models with Confident Reasoning

Large language models (LLMs) have shown impressive performance by generating reasoning paths before final answers, but learning such a reasoning path requires costly human supervision. To address this issue, recent studies have explored self-training methods that improve reasoning capabilities using pseudo-labels generated by the LLMs themselves. Among these, confidence-based self-training fine-tunes LLMs to prefer reasoning paths with high-confidence answers, where confidence is estimated via majority voting. However, such methods exclusively focus on the quality of the final answer and may ignore the quality of the reasoning paths, as even an incorrect reasoning path leads to a correct answer by chance. Instead, we advocate the use of reasoning-level confidence to identify high-quality reasoning paths for self-training, supported by our empirical observations. We then propose a new self-training method, CORE-PO, that fine-tunes LLMs to prefer high-COnfidence REasoning paths through Policy Optimization. Our experiments show that CORE-PO improves the accuracy of outputs on four in-distribution and two out-of-distribution benchmarks, compared to existing self-training methods.

==> 3_2_related_work.tex <==
\section{Related works} \label{sec:related}


\noindent \textbf{Confidence measures for LLMs.} Large language models (LLMs) often generate incorrect outputs due to hallucinations, which highlights the importance of estimating confidence in their outputs. To this end, several methods have been proposed, e.g., self-consistency \citep{wang2023selfconsistency}, semantic entropy over the sequences with the same semantics \citep{farquhar2024detecting}, or $\text{P(True)}$ \citep{kadavath2022languagemodelsmostlyknow}. In addition, \citet{lin-etal-2024-contextualized} propose computing confidence using the likelihoods of important tokens that determine semantics of the sequence. Recently, several studies have shown that measures based on $\text{P(True)}$ or the likelihoods of important tokens can be utilized to estimate the confidence in reasoning \citep{becker2024cyclesthoughtmeasuringllm,taubenfeld2025confidence,razghandi2025cer}. %Although such confidence measures have mainly been applied to single-statement factuality checks, recent studies have shown that measures based on $\text{P(True)}$ or the likelihoods of important tokens can be utilized to estimate the confidence in reasoning \citep{becker2024cyclesthoughtmeasuringllm,taubenfeld2025confidence,razghandi2025cer}.


\noindent \textbf{Inference-time scaling methods for LLMs.} Inference-time scaling methods improve the quality of LLM outputs by self-assessing multiple generated outputs. Among them, self-consistency-based method \citep{wang2023selfconsistency} selects the most frequent answer obtained through the majority voting. Other approaches include tree-of-thoughts \citep{yao2023tree}, which expands the search space over intermediate steps, and self-refinement inference \citep{madaan2023self}, which iteratively refine outputs using the LLM itself. In addition, \citet{taubenfeld2025confidence} recently proposed incorporating confidence scores on reasoning paths into the self-consistency method and shown notable performance improvements.

 
%\noindent \textbf{Training of reasoning for LLMs.} To enhance reasoning abilities, LLMs have been initially fine-tuned using various supervision signals. A straightforward approach is supervised fine-tuning (SFT) using human-annotated reasoning paths \citep{xxx}. While effective, SFT requires high-quality reasoning annotations, which are expensive to collect. To alleviate this, several studies propose reinforcement learning methods that rely solely on ground-truth answers, using answer-level accuracy as the reward signal \citep{xxx}. In addition, several studies propose to incorporate process-level rewards computed by external models that assess the quality of intermediate reasoning steps \citep{xxx}.


\noindent \textbf{Other self-training approaches for LLMs.} We further describe self-training methods derived from inference-time scaling techniques that do not rely on confidence scores. First, \citet{kumar2024self-rewarding} propose using linguistic assessments of output quality, e.g., assigning high scores to outputs that exhibit expert-level knowledge, as reward signals for fine-tuning LLMs. Next, \citet{ranaldi2024self} propose using outputs obtained from self-refinement inference \citep{madaan2023self}, as these outputs typically exhibit higher quality than the initial outputs. Finally, \citet{zhang2024chain} leverage preference signals over intermediate reasoning steps derived from tree-of-thoughts inference \citep{yao2023tree}.


